ForTress: Bringing Assurance and Determinism for LLM-Driven Fortran-to-Python Translation

Modernizing mature scientific software from Fortran to Python can improve accessibility and integration with modern computing tools, but manual rewriting is expensive. Large language models (LLMs) make translation more practical, yet generated code can pass regression tests while violating source-language semantics, and contextual corrections may not persist across subsequent translations. We present ForTress, which solidifies recurring LLM translation decisions into guarded executable rules for deterministic reuse and provides semantic assurance for a non-trivial subset of these rules. Its LLM-assisted auditing process expresses universally quantified preservation obligations over mechanized Fortran and Python semantics in Lean. Human experts review semantic fidelity and correspondence with production rules, and Lean's kernel checks proofs and refutations under explicit assumptions. These audit records expose the conditions either supporting correctness or identifying failure cases. We evaluate ForTress on 17 benchmarks from 15 scientific software spanning diverse domains. The translated programs achieve bitwise-identical with native Fortran on all evaluated tests under the recorded execution and initialization configurations. Against these software, ForTress accumulates 193 executable rules and 188 audit records, of which 121 have checked soundness proofs, including 31 established after counterexample-guided refinement. Cross-software reuse exceeds 90% for 14 of the 15 software. Even with additional assurance and determinism, the LLM usage cost is 44.2% lower than direct LLM translation.

==> code-style-d.tex <==
% code-style-d.tex -- compatibility loader for the selected dafny25 preset.
% Preamble: \input{code-style-d}. Existing [style=styleD] blocks keep working.
% The user's code-styles.tex v2 is unchanged. No global \lstset is installed.
% dafny25: orange bold keywords, green comments, 0-based line numbers,
% top/bottom rules, 9pt code, and the preset's original fixed character pitch.
\ifdefined\CodeStyleDLoaded\endinput\fi
\let\CodeStyleDLoaded\relax
\def\CodeStyleDTemplateVersion{2-dafny25}

\RequirePackage{xcolor}
\RequirePackage{listings}
\RequirePackage{amsmath}
\ifdefined\mathbb\else\RequirePackage{amsfonts}\fi

% Avoid loading the user's presets twice if main.tex already loads them.
\ifcsname lststy@dafny25$\endcsname\else
  \input{code-styles}
\fi

\lstdefinestyle{paperDafny25}{
  style=dafny25,
  % Preserve the selected preset's typography; clear unrelated global settings.
  basicstyle=\normalfont\small\ttfamily\color{black},
  columns=fixed,
  basewidth=0.6em,
  keepspaces=true,
  keywordstyle=\bfseries\color{dafnyKw},
  keywordstyle=[2]{\bfseries\color{dafnyKw}},
  keywordstyle=[3]{\bfseries\color{dafnyKw}},
  keywordstyle=[4]{\normalfont\small\ttfamily\color{black}},
  keywordstyle=[5]{\normalfont\small\ttfamily\color{black}},
  identifierstyle=\color{black},
  stringstyle=\color{black},
  commentstyle=\color{dafnyCm},
  showspaces=false,
  showtabs=false,
  showstringspaces=false,
  numbers=left,
  numberstyle=\normalfont\tiny\color{black},
  stepnumber=1,
  numbersep=10pt,
  firstnumber=0,
  numberblanklines=true,
  frame=tb,
  rulecolor=\color{black},
  framerule=0.4pt,
  framesep=3pt,
  xleftmargin=10pt,
  xrightmargin=10pt,
  backgroundcolor={},
  resetmargins=false,
  linewidth=\linewidth,
  lineskip=0pt,
  aboveskip=6pt,
  belowskip=2pt,
  breaklines=true,
  breakatwhitespace=false,
  breakautoindent=true,
  breakindent=1em,
  prebreak={},
  postbreak={},
  mathescape=false,
  texcl=false,
  escapechar={},
  escapeinside={(*@}{@*)},
  extendedchars=true,
  % Extend the preset's Unicode table for the existing Lean excerpts.
  % Do not retain epr26's coloured ASCII operators or its type palette.
  literate=
    {→}{{$\rightarrow$}}1 {←}{{$\leftarrow$}}1
    {⇒}{{$\Rightarrow$}}1 {⟹}{{$\Longrightarrow$}}3
    {↦}{{$\mapsto$}}1 {≤}{{$\le$}}1 {≥}{{$\ge$}}1
    {≠}{{$\neq$}}1 {∀}{{$\forall$}}1 {∃}{{$\exists$}}1
    {λ}{{$\lambda$}}1 {∧}{{$\wedge$}}1 {∨}{{$\vee$}}1
    {¬}{{$\neg$}}1 {∅}{{$\emptyset$}}1 {∪}{{$\cup$}}1
    {∈}{{$\in$}}1 {⊔}{{$\sqcup$}}1 {⊢}{{$\vdash$}}1
    {⊥}{{$\bot$}}1 {α}{{$\alpha$}}1 {τ}{{$\tau$}}1
    {Γ}{{$\Gamma$}}1 {σ}{{$\sigma$}}1
    {ℝ}{{$\mathbb{R}$}}1 {ℤ}{{$\mathbb{Z}$}}1
    {ℕ}{{$\mathbb{N}$}}1
    {⌊}{{$\lfloor$}}1 {⌋}{{$\rfloor$}}1
    {⌈}{{$\lceil$}}1 {⌉}{{$\rceil$}}1
    {⟨}{{$\langle$}}1 {⟩}{{$\rangle$}}1
}
% Backward-compatible name: old source files need no mass style-name changes.
\lstdefinestyle{styleD}{style=paperDafny25}
% For real tool output, if needed later. Do not label proof signatures as output.
\lstdefinestyle{paperDafny25out}{
  style=paperDafny25, language={}, basicstyle=\normalfont\footnotesize\ttfamily,
  numbers=none, frame=none, xleftmargin=20pt,
  aboveskip=6pt, belowskip=6pt
}

% Language aliases only provide tokenization; the style supplies the palette.
\lstdefinelanguage{PythonD}[3]{Python}{}
\lstdefinelanguage{LeanD}{
  morekeywords={def,theorem,lemma,example,noncomputable,inductive,structure,
    where,if,then,else,let,in,match,with,fun,by,have,show,from,exact,
    intro,intros,obtain,cases,rcases,rw,simp,simpa,decide,rfl,
    namespace,end,open,import,variable,variables,instance,deriving,
    private,protected,abbrev,axiom,opaque,constant,do,return},
  morekeywords=[2]{Type,Prop,Sort,Nat,Int,Real,Bool},
  morekeywords=[3]{some,none,true,false},
  morekeywords=[4]{Option,List,Array,Fin},
  sensitive=true,
  alsoletter={'},
  morecomment=[l]{--},
  morecomment=[n]{/-}{-/},
  morestring=[b]"
}


==> code-styles.tex <==
%% code-styles.tex  (v2)
%% listings presets that reproduce the code figures of specific OOPSLA papers.
%%
%% Every preset is named after ONE paper. Its header gives the paper, the DOI,
%% the figure it reproduces, and the parameters measured from the published PDF
%% (font, size, line spacing, character pitch, colours, numbers, rules).
%%
%% Usage, in the preamble of an acmart paper:   \input{code-styles}
%% then  \begin{lstlisting}[style=dafny25, language=Dafny] ... \end{lstlisting}
%%
%% Only listings + xcolor are needed (acmart already loads xcolor). Three presets
%% switch the typewriter font *inside the listing only*, as their papers did:
%% sse26 and vis24 use Bera Sans Mono, iac24 uses newtxtt (both in TeX Live).
%% To stay on acmart's Inconsolata, delete the \renewcommand*{\ttdefault}{...}
%% part of their basicstyle.
%%
%% Each preset also sets the language of its figure; override it after the
%% style, e.g.  [style=dafny25, language=Java].
%%
%% Several papers use the listings default columns=fixed (0.6em grid), which
%% letter-spaces Inconsolata (0.5em wide). The presets keep that look on purpose;
%% append  style=tight  to any listing to remove it:  [style=dafny25, style=tight]
%%
%% Line spacing note (measured in acmart): a listing without a frame gets the
%% size's \baselineskip + ~1pt (\small: 12pt); with any frame it gets exactly the
%% size's \baselineskip (\small: 11pt).  The `lineskip' values below compensate.

\usepackage{listings}

%% ======================================================================
%% Helpers
%% ======================================================================
%% NB: listings' own default is commentstyle=\itshape; Inconsolata has no italic,
%% so every preset below sets commentstyle explicitly.
\lstdefinestyle{tight}{columns=fullflexible, keepspaces=true}

%% whole-line background: put (*@\hlline{colour}@*) at the very start of a line
\newcommand{\hlline}[1]{%
  \makebox[0pt][l]{\color{#1}\rule[-0.3\baselineskip]{\linewidth}{\baselineskip}}}
%% background behind one token or formula: (*@\hlbox{colour}{...}@*)
%% (plain \colorbox with 3pt padding, as measured in sse26; change \hlboxsep)
\newlength{\hlboxsep}\setlength{\hlboxsep}{3pt}
\newcommand{\hlbox}[2]{{\setlength{\fboxsep}{\hlboxsep}\colorbox{#1}{#2}}}

%% Bera Sans Mono is used at 85% (beramono's usual scaled=0.85) by sse26/vis24.
%% The font is switched by redefining \ttdefault *inside* the listing, so that
%% listings still treats it as typewriter and prints '-' as a hyphen, not a minus.
\makeatletter\providecommand*{\fvm@Scale}{0.85}\makeatother

%% ======================================================================
%% Languages (keyword sets follow what is highlighted in each figure)
%% ======================================================================
\lstdefinelanguage{Dafny}{
  morekeywords={method,function,predicate,lemma,returns,requires,ensures,modifies,
    reads,decreases,invariant,assert,assume,var,if,then,else,while,forall,exists,
    old,class,datatype,ghost,return,this,new,null,true,false,
    int,nat,real,bool,seq,set,map,array,string,uint64},
  sensitive=true, morecomment=[l]{//}, morecomment=[s]{/*}{*/}, morestring=[b]",
}
\lstdefinelanguage{Forge}{
  morekeywords={abstract,sig,one,lone,some,no,all,extends,pfunc,func,set,Int,pred,
    fun,or,and,implies,not,iff,in,let,disj,var,always,eventually,test,expect,run,
    check,example,is,sat,unsat,theorem},
  sensitive=true, morecomment=[l]{--}, morecomment=[l]{//}, morecomment=[s]{/*}{*/},
}
\lstdefinelanguage{Rust}{
  morekeywords={as,async,await,break,const,continue,crate,dyn,else,enum,extern,fn,
    for,if,impl,in,let,loop,match,mod,move,mut,pub,ref,return,self,Self,static,
    struct,super,trait,type,unsafe,use,where,while},
  morekeywords=[2]{bool,char,f32,f64,i8,i16,i32,i64,i128,isize,str,u8,u16,u32,u64,
    u128,usize},
  morekeywords=[3]{Box,Option,Result,Some,None,Ok,Err,Vec,String},
  sensitive=true, morecomment=[l]{//}, morecomment=[s]{/*}{*/}, morestring=[b]",
}
\lstdefinelanguage{HaskellCore}{   % only the keywords ChatLSP's listing sets in bold
  morekeywords={let,in,where,case,of,if,then,else,do,data,type,module,import},
  sensitive=true, morecomment=[l]{--}, morecomment=[s]{\{-}{-\}}, morestring=[b]",
}
\lstdefinelanguage{Viper}{
  morekeywords={method,function,predicate,field,returns,requires,ensures,invariant,
    var,havoc,inhale,exhale,assert,assume,fold,unfold,acc,if,else,while,
    Int,Bool,Ref,Perm},
  sensitive=true, morecomment=[l]{//},
}
\lstdefinelanguage{Coq}{
  morekeywords={Variable,Definition,Fixpoint,Inductive,Record,Lemma,Theorem,Proof,
    Qed,match,with,end,let,in,do,fun,forall,exists,if,then,else,return},
  sensitive=true, morecomment=[s]{(*}{*)},
}
\lstdefinelanguage{Puppet}{
  morekeywords={package,file,service,exec,class,define,node,include,require,user},
  sensitive=true, morecomment=[l]{\#}, morestring=[b]", morestring=[b]',
}
\lstdefinelanguage{Ansible}{
  sensitive=true, morecomment=[l]{\#}, morestring=[b]", morestring=[b]',
}
\lstdefinelanguage{JSONmut}{          % JSON plus // comments, as in Prunario
  sensitive=true, morestring=[b]", morecomment=[l]{//},
}
\lstdefinelanguage{FiberAsm}{         % the x86 snippet of WasmFX, Fig. 5b
  morekeywords={push,pop,mov,ret,call,jmp},
  sensitive=true, morecomment=[l]{//},
}
\lstdefinelanguage{RhombusDSL}{
  sensitive=true, morestring=[b]", morecomment=[l]{//},
}

%% ======================================================================
%% dafny25 -- E. Mugnier, Y. Zhou, R. Jhala, M. Coblenz.
%%   On the Impact of Formal Verification on Software Development.
%%   PACMPL 9(OOPSLA2), Article 403, 2025.  doi:10.1145/3763181
%%   Reproduces Fig. 1 (p. 403:3); Figs. 2-3 use the same style.
%%   Measured: Inconsolata 9pt (\small) on 11pt; columns=fixed (0.6em pitch,
%%   letter-spaced); keywords bold #E67300; comments #009900; numbers \tiny
%%   Libertine, black, from 0, numbersep 10pt; frame=tb 0.4pt; listing indented
%%   10pt on both sides; tool output below the bottom rule in \footnotesize.
%% ======================================================================
\definecolor{dafnyKw}{HTML}{E67300}
\definecolor{dafnyCm}{HTML}{009900}
\lstdefinestyle{dafny25}{
  language=Dafny,
  basicstyle=\ttfamily\small,                   % with a frame: 9pt on 11pt
  columns=fixed,
  keywordstyle=\bfseries\color{dafnyKw},
  commentstyle=\color{dafnyCm},
  showstringspaces=false, upquote=true, tabsize=2,
  numbers=left, numberstyle=\tiny, numbersep=10pt, firstnumber=0,
  frame=tb, framerule=0.4pt, framesep=3pt,
  xleftmargin=10pt, xrightmargin=10pt,
  aboveskip=6pt, belowskip=2pt,
  escapeinside={(*@}{@*)}, extendedchars=true,
  literate={≤}{{$\le$}}1 {≥}{{$\ge$}}1 {⟹}{{$\Longrightarrow$}}3 {∧}{{$\wedge$}}1
           {∨}{{$\vee$}}1 {¬}{{$\neg$}}1 {≠}{{$\neq$}}1,
}
%% the verifier message typeset under the bottom rule (no numbers, no frame).
%% The paper highlights `this'/`return' in it because it reuses language=Dafny;
%% add language=Dafny to reproduce that, or keep the default (plain) below.
\lstdefinestyle{dafny25out}{
  style=dafny25, language={}, basicstyle=\ttfamily\footnotesize, lineskip=0pt,
  numbers=none, frame=none, xleftmargin=20pt, aboveskip=6pt, belowskip=6pt,
}

%% ======================================================================
%% enumo23 -- A. Pal, B. Saiki, R. Tjoa, C. Richey, A. Zhu, O. Flatt,
%%   M. Willsey, Z. Tatlock, C. Nandi.
%%   Equality Saturation Theory Exploration a la Carte.
%%   PACMPL 7(OOPSLA2), Article 258, 2023.  doi:10.1145/3622834
%%   Reproduces Fig. 7 (p. 258:17).
%%   Measured: Inconsolata 8pt (\footnotesize) on 11pt; natural pitch; keywords
%%   bold black; numbers \footnotesize Libertine black, numbersep 10pt; no frame;
%%   maths escapes ($\mathcal{G}$).
%% ======================================================================
\lstdefinestyle{enumo23}{
  language=Python,
  basicstyle=\ttfamily\footnotesize,
  columns=fullflexible, keepspaces=true,
  keywordstyle=\bfseries,
  commentstyle=\color{black!60},          % no comment in the figure: our choice
  showstringspaces=false, upquote=true,
  numbers=left, numberstyle=\footnotesize, numbersep=10pt,
  xleftmargin=12pt, aboveskip=6pt, belowskip=6pt,
  mathescape=true, escapeinside={(*@}{@*)},
}

%% ======================================================================
%% forge24 -- T. Nelson, B. Greenman, S. Prasad, et al.
%%   Forge: A Tool and Language for Teaching Formal Methods.
%%   PACMPL 8(OOPSLA1), Article 116, 2024.  doi:10.1145/3649833
%%   Reproduces Fig. 1 (p. 116:7).
%%   Measured: Inconsolata 9pt (\small) on 12pt; columns=fixed (letter-spaced);
%%   keywords bold black; no numbers, no frame, flush with the text margin.
%% ======================================================================
\lstdefinestyle{forge24}{
  language=Forge,
  basicstyle=\ttfamily\small,
  columns=fixed,
  keywordstyle=\bfseries, commentstyle={},
  showstringspaces=false, upquote=true,
  numbers=none, frame=none, xleftmargin=0pt,
  aboveskip=6pt, belowskip=6pt, escapeinside={(*@}{@*)},
}

%% ======================================================================
%% chatlsp24 -- A. Blinn, X. Li, J. H. Kim, C. Omar.
%%   Statically Contextualizing Large Language Models with Typed Holes.
%%   PACMPL 8(OOPSLA2), Article 288, 2024.  doi:10.1145/3689728
%%   Reproduces the API listing on p. 288:23.
%%   Measured: Inconsolata 9pt on 11pt; columns=fixed (letter-spaced); keywords
%%   bold black; comments grey #7F807F; frame=single 0.4pt black spanning the
%%   full text width; no numbers.
%% ======================================================================
\definecolor{chatCm}{HTML}{7F807F}
\lstdefinestyle{chatlsp24}{
  language=HaskellCore,
  basicstyle=\ttfamily\small,                   % with a frame: 9pt on 11pt
  columns=fixed,
  keywordstyle=\bfseries, commentstyle=\color{chatCm},
  showstringspaces=false, upquote=true,
  numbers=none,
  frame=single, framerule=0.4pt, framesep=3pt, rulecolor=\color{black},
  xleftmargin=3.4pt, xrightmargin=3.4pt,
  aboveskip=8pt, belowskip=8pt, escapeinside={(*@}{@*)}, extendedchars=true,
  literate={→}{{$\rightarrow$}}1,
}

%% ======================================================================
%% epr26 -- N. V. Lewchenko, K. Kim, B.-Y. E. Chang, G. Kaki.
%%   Effectively Propositional Higher-Order Functional Programming.
%%   PACMPL 10(OOPSLA1), Article 151, 2026.  doi:10.1145/3798259
%%   Reproduces Fig. 6 (p. 151:21), set with minted's default Pygments theme.
%%   Measured: Inconsolata 9pt on 11pt; natural pitch; keywords bold #008000;
%%   primitive types bold #B00040; builtins #008000; type names bold #0000FF;
%%   function names #0000FF; operators #666666; no numbers, no frame.
%%   listings cannot find type/function names by context: list them per listing
%%   with  morekeywords={[4]Heap,State}  (types) and  morekeywords={[5]init}  (fns);
%%   Pygments colours a type name only in annotation position, listings everywhere.
%% ======================================================================
\definecolor{pgKw}{HTML}{008000}
\definecolor{pgTy}{HTML}{B00040}
\definecolor{pgNm}{HTML}{0000FF}
\definecolor{pgOp}{HTML}{666666}
\definecolor{pgCm}{HTML}{3D7B7B}
\definecolor{pgSt}{HTML}{BA2121}
\lstdefinestyle{epr26}{
  language=Rust,
  basicstyle=\ttfamily\small, lineskip=-1pt,  % minted at \small: 9pt on 11pt
  columns=fullflexible, keepspaces=true,
  keywordstyle=[1]{\bfseries\color{pgKw}},
  keywordstyle=[2]{\bfseries\color{pgTy}},
  keywordstyle=[3]{\color{pgKw}},
  keywordstyle=[4]{\bfseries\color{pgNm}},
  keywordstyle=[5]{\color{pgNm}},
  commentstyle=\color{pgCm}, stringstyle=\color{pgSt},
  showstringspaces=false, upquote=true,
  numbers=none, frame=none, xleftmargin=0pt,
  aboveskip=6pt, belowskip=6pt, escapeinside={(*@}{@*)},
  literate={=}{{\color{pgOp}=}}1 {<}{{\color{pgOp}<}}1 {>}{{\color{pgOp}>}}1
           {!}{{\color{pgOp}!}}1 {&}{{\color{pgOp}\&}}1,
}

%% ======================================================================
%% prunario26 -- M. Kim, S. So, H. Oh.
%%   Prunario: Testing Autonomous Driving Systems by Pruning Likely Redundant
%%   Scenarios.  PACMPL 10(OOPSLA1), Article 154, 2026.  doi:10.1145/3798262
%%   Reproduces the mutated-scenario listing on p. 154:16.
%%   Measured: Inconsolata 6pt (\tiny) on 7.1pt; columns=fixed (letter-spaced);
%%   strings #0000FF; numbers \tiny black outside the frame; frame=single 0.4pt;
%%   background gray!5; changed lines green!20 / red!20 (use \hlline).
%% ======================================================================
\colorlet{prAdd}{green!20}
\colorlet{prDel}{red!20}
\lstdefinestyle{prunario26}{
  language=JSONmut,
  basicstyle=\ttfamily\tiny,                    % with a frame: 6pt on 7pt
  columns=fixed,
  stringstyle=\color{blue}, commentstyle={},
  showstringspaces=false, upquote=true,
  numbers=left, numberstyle=\tiny, numbersep=8.3pt,
  frame=single, framerule=0.4pt, framesep=3pt, rulecolor=\color{black},
  backgroundcolor=\color{gray!5},
  xleftmargin=11pt, xrightmargin=2.6pt,
  aboveskip=6pt, belowskip=6pt, escapeinside={(*@}{@*)},
}

%% ======================================================================
%% sse26 -- H. Ling, T. Dardinier, E. Arlt, P. Mueller.
%%   Sound State Encodings in Translational Separation Logic Verifiers.
%%   PACMPL 10(OOPSLA2), Article 330, 2026.  doi:10.1145/3839462
%%   Reproduces Fig. 1b (p. 330:2).
%%   Measured: Bera Sans Mono at 85% of \footnotesize (6.8pt) on 10pt, maths at
%%   8pt; keywords bold #4069E0; comments #009900; frame=tb per column, 3-space
%%   indentation; no numbers; formulas as maths in \colorbox'es (yellow,
%%   blue!20, green!25, red!20; use \hlbox).
%% ======================================================================
\definecolor{sseKw}{HTML}{4069E0}
\definecolor{sseCm}{HTML}{009900}
\definecolor{sseY}{rgb}{1,0.981,0.76}
\colorlet{sseB}{blue!20}
\colorlet{sseG}{green!25}
\colorlet{sseR}{red!20}
\lstdefinestyle{sse26}{
  language=Viper,
  basicstyle=\renewcommand*{\ttdefault}{fvm}\ttfamily\footnotesize, % Bera 85%: 6.8pt
  columns=fixed,
  keywordstyle=\bfseries\color{sseKw}, commentstyle=\color{sseCm},
  showstringspaces=false, upquote=true,
  numbers=none, frame=tb, framerule=0.4pt, framesep=3pt,
  xleftmargin=0pt, aboveskip=6pt, belowskip=6pt,
  escapeinside={(*@}{@*)}, extendedchars=true,
  literate={¬}{{$\neg$}}1 {↦}{{$\mapsto$}}1,
}

%% ======================================================================
%% wasmfx23 -- L. Phipps-Costin, A. Rossberg, A. Guha, D. Leijen,
%%   D. Hillerstroem, K. Sivaramakrishnan, M. Pretnar, S. Lindley.
%%   Continuing WebAssembly with Effect Handlers.
%%   PACMPL 7(OOPSLA2), Article 238, 2023.  doi:10.1145/3622814
%%   Reproduces Fig. 5 (p. 238:18).
%%   Measured: Linux Biolinum (acmart \sffamily) 9pt, proportional; keywords
%%   bold; comments italic; '-' printed as a minus sign; no numbers, no frame.
%% ======================================================================
\lstdefinestyle{wasmfx23}{
  language=Rust,
  basicstyle=\sffamily\small,
  columns=fullflexible, keepspaces=true,
  keywordstyle=\bfseries, keywordstyle=[2]{}, keywordstyle=[3]{},
  commentstyle=\itshape,
  showstringspaces=false,
  numbers=none, frame=none, xleftmargin=14pt,
  aboveskip=6pt, belowskip=6pt, escapeinside={(*@}{@*)},
}   % '-' comes out as a minus sign automatically (listings does that for
    % non-typewriter fonts), exactly as in the paper

%% ======================================================================
%% iac24 -- G.-P. Drosos, T. Sotiropoulos, G. Alexopoulos, D. Mitropoulos, Z. Su.
%%   When Your Infrastructure Is a Buggy Program: Understanding Faults in
%%   Infrastructure as Code Ecosystems.
%%   PACMPL 8(OOPSLA2), Article 359, 2024.  doi:10.1145/3689799
%%   Reproduces Fig. 2 (p. 359:4): two programs side by side.
%%   Measured: newtxtt 6pt (\tiny) on 8pt; natural pitch; keywords bold; strings
%%   #0000FF; numbers \tiny Libertine black, numbersep 10pt; no frame.
%% ======================================================================
\lstdefinestyle{iac24}{
  basicstyle=\renewcommand*{\ttdefault}{newtxtt}\ttfamily\tiny, % newtxtt
  columns=fullflexible, keepspaces=true,
  keywordstyle=\bfseries, stringstyle=\color{blue}, commentstyle={},
  showstringspaces=false, upquote=true,
  numbers=left, numberstyle=\tiny, numbersep=10pt,
  frame=none, xleftmargin=12pt, aboveskip=4pt, belowskip=4pt,
  escapeinside={(*@}{@*)},
}

%% ======================================================================
%% bingraph24 -- Y. Zhang, Y. Shi, X. Zhang.
%%   Learning Abstraction Selection for Bayesian Program Analysis.
%%   PACMPL 8(OOPSLA1), Article 128, 2024.  doi:10.1145/3649845
%%   Reproduces Fig. 1 (p. 128:3): one program in two columns, numbering
%%   continued in the second column (firstnumber=27).
%%   Measured: Inconsolata 7pt (\scriptsize) on 9pt; natural pitch; keywords
%%   #C10846 (not bold); comments #0000FF; numbers \scriptsize Libertine black.
%% ======================================================================
\definecolor{bgKw}{HTML}{C10846}
\lstdefinestyle{bingraph24}{
  language=Java,
  basicstyle=\ttfamily\scriptsize,
  columns=fullflexible, keepspaces=true,
  keywordstyle=\color{bgKw}, commentstyle=\color{blue},
  showstringspaces=false, upquote=true,
  numbers=left, numberstyle=\scriptsize, numbersep=10pt,
  frame=none, xleftmargin=14pt, aboveskip=4pt, belowskip=4pt,
  escapeinside={(*@}{@*)},
}

%% ======================================================================
%% vis24 -- Z. Yang, J. Shirako, V. Sarkar.  Fully Verified Instruction
%%   Scheduling.  PACMPL 8(OOPSLA2), Article 299, 2024.  doi:10.1145/3689739
%%   Reproduces the Coq listing on p. 299:17.
%%   Measured: Bera Sans Mono 7.2pt on 10pt; keywords bold #008700; comments
%%   #878787; numerals bold #0000DE; no numbers, no frame.
%% ======================================================================
\definecolor{visKw}{HTML}{008700}
\definecolor{visCm}{HTML}{878787}
\definecolor{visNum}{HTML}{0000DE}
\lstdefinestyle{vis24}{
  language=Coq,
  basicstyle=\renewcommand*{\ttdefault}{fvm}\ttfamily\fontsize{8.47}{9.03}\selectfont, % 7.2pt
  columns=fixed,
  keywordstyle=\bfseries\color{visKw}, commentstyle=\color{visCm},
  alsoletter={0123456789},                 % numerals become tokens ...
  morekeywords={[2]0,1,2,3,4,5,6,7,8,9},   % ... so stand-alone ones can be styled
  keywordstyle={[2]\bfseries\color{visNum}},
  showstringspaces=false, upquote=true,
  numbers=none, frame=none, xleftmargin=0pt,
  aboveskip=6pt, belowskip=6pt, escapeinside={(*@}{@*)},
}

%% ======================================================================
%% rhombus23 -- M. Flatt, T. Allred, N. Angle, et al.
%%   Rhombus: A New Spin on Macros without All the Parentheses.
%%   PACMPL 7(OOPSLA2), Article 242, 2023.  doi:10.1145/3622818
%%   Reproduces Fig. 13 (p. 242:23), Racket/Scribble colours.
%%   Measured: Inconsolata 8pt on 10pt; natural pitch; identifiers #262680;
%%   strings and numerals #218C21; comments #C2731F; parentheses #843D24.
%% ======================================================================
\definecolor{rhId}{HTML}{262680}
\definecolor{rhSt}{HTML}{218C21}
\definecolor{rhCm}{HTML}{C2731F}
\definecolor{rhPn}{HTML}{843D24}
\lstdefinestyle{rhombus23}{
  language=RhombusDSL,
  basicstyle=\ttfamily\footnotesize, lineskip=-1pt,
  columns=fullflexible, keepspaces=true,
  identifierstyle=\color{rhId}, stringstyle=\color{rhSt}, commentstyle=\color{rhCm},
  alsoletter={0123456789}, morekeywords={[2]0,1,2,3,4,5,6,7,8,9},
  keywordstyle={[2]\color{rhSt}},
  showstringspaces=false, upquote=true,
  numbers=none, frame=none, xleftmargin=15pt,
  aboveskip=6pt, belowskip=6pt, escapeinside={(*@}{@*)},
  literate={(}{{\color{rhPn}(}}1 {)}{{\color{rhPn})}}1,
}

%% ======================================================================
%% Generic helpers kept from v1
%% ======================================================================
%% inline code at text size; add language=... for bold keywords
\lstdefinestyle{inline}{basicstyle=\ttfamily, columns=fullflexible, keepspaces=true,
  keywordstyle=\bfseries, showstringspaces=false, upquote=true}
\providecommand{\code}{\lstinline[style=inline]}

